EPIC: Efficient Position-Independent Caching for Serving Large Language Models

Large Language Models (LLMs) show great capabilities in a wide range of applications, but serving them efficiently becomes increasingly challenging as requests (prompts) become more complex. Context caching improves serving performance by reusing Key-Value (KV) vectors, the intermediate representations of tokens that are repeated across requests. However, existing context caching requires exact prefix matches across requests, limiting reuse cases in settings such as few-shot learning and retrieval-augmented generation, where immutable content (e.g., documents) remains unchanged across requests but is preceded by varying prefixes. Position-Independent Caching (PIC) addresses this issue by enabling modular reuse of the KV vectors regardless of prefixes. We formalize PIC and advance prior work by introducing EPIC, a serving system incorporating our new LegoLink algorithm, which mitigates the inappropriate "attention sink" effect at every document beginning, to maintain accuracy with minimal computation. Experiments show that EPIC achieves up to 8x improvements in Time-To-First-Token (TTFT) and 7x throughput gains over existing systems, with negligible or no accuracy loss.

==> figs/fig-eval-kvsplit.tex <==
\begin{figure}[thbp]
    \centering
    \includegraphics[width=\linewidth]{figs/figs/fig-eval-kvsplit.pdf}
    \caption{The axes, legends, and data points in this figure follow the same definitions as those in Figure~\ref{fig-eval-e2e}, with one key difference: the second column represents results from the Mistral model using fixed-size token chunks (512 tokens per chunk). We only show the results of one model and two datasets due to the page limitation.}
    \label{fig-eval-kvsplit}
\end{figure}

==> sections/impl.tex <==
\section{Implementation}
\label{sec-impl}

%\system\ has three core components, \textit{KVGen}, \textit{KVStore} and \textit{KVLink}, together with an auxiliary component \textit{KVSplit}.

We implement \system\ based on vLLM 0.4.1~\cite{kwon2023vllm}, with 2K lines of code in Python. We incorporate the four PIC recomputation algorithms presented in Section~\ref{sec-algo}. We port CacheBlend from their public repository\footnote{https://github.com/YaoJiayi/CacheBlend. Accessed on Sep 2024.}.

%\footnote{https://github.com/YaoJiayi/CacheBlend}

%with 1k for \textit{KVSplit} data pipeline, 100 for API alternation including generate\_context\_cache, extended version of chat\_completion. 400 (?) for kvdb. 500 for core algorithm logic. 500 for glue code.}
We implement \textit{KVSplit} as a standalone component independent of \system.
%enabling users to incorporate custom splitting methods by overriding the \texttt{\_static\_token\_split} method.
%
We provide two basic implementations: one splits tokens based on semantic boundaries (e.g., sentence, paragraph, or passage), while the other uses fixed-size chunks (e.g., 512 tokens). Users can choose the desired granularity of chunks and \textbf{optionally} employ \textit{KVSplit}; they can also integrate external tools, such as Retrieval-Augmented Generation (RAG) for chunking. Improved chunking techniques correlate with enhanced accuracy (Figure~\ref{fig-eval-kvsplit}) and greater reusability.

%In the following experiment, we use semantic-based splitting method by default. \ys{move this to eval}

% Second, \textit{KVSplit} offers helper tools, such as pattern and semantic matching methods, to facilitate the rewriting of \texttt{\_static\_token\_split}.
% Users can also integrate external tools, like Retrieval-Augmented Generation (RAG), provided the input is a sequence of static tokens and the output is a list of token chunks.
%\ys{For users of explicit CC APIs, it is unclear why and how they should use KVSplit. Also, I think KVSplit is not a core part of \system\ because for explicit API usage, this is entirely done by users.}


%We implement a \textit{KVStore} that manages the storage and rMooncake~\cite{qin2407mooncake}.
We implement the \textit{KVStore} based on vLLM's original memory management and prefix caching subsystem.
%
We make the following changes.
First, we add a cache-ID-based indexing mechanism using the sequence group ID as the cache ID.
Second, since the original vLLM manages historical KV cache residing in HBM only, we extend it to include DRAM and local filesystem, akin to Mooncake~\cite{qin2407mooncake}.
%
Third, we modify the scheduler to retain block tables and memory for context caching requests.
%
%\ys{isn't the above feature already implemented in vllm prefix caching?}
%
We also implement helper APIs that allow users to manage the lifecycle of KV cache, such as \texttt{expire\_cache(cache\_id)}.
%
As building a highly efficient \textit{KVStore} is not the core focus of this paper, we build a minimal working system.
\system\ can use external \textit{KVStore} systems like LMCache~\cite{lmcache-github}, which we leave for future work.

We implement \textit{KVGen} as a standalone module that handles CC APIs.
%
%invokes the underlying inference engine with the maximum generated tokens parameter set to one. This function also interacts with \textit{KVStore}.
%
% resides on the same generates KV cache for static token chunks using an inference engine and stores them in \textit{KVStore}. Both \textit{KVGen} and \textit{KVLink} replace the prefill stage in the inference engine with a new prefill process.\
% Developer es can replace the new prefill provided by \textit{KVGen} component with different algorithms, such as those that embed information into the generated KV cache, improving the linking process. Currently, we use the ordinary prefill process as the prefill implementation in \textit{KVGen}.
%
%
We implement \textit{KVLink} as a parallel module of the original prefill. First, we adapt the model architecture to support masked attention across tokens scattered in different positions. Second, we modify the attention backends to handle data placement, movement, and the computational steps required by the preceding algorithm. These changes ensure efficient recomputation and accurate linking between static and dynamic tokens.

\system\ offers APIs similar to those in Kimi~\cite{kimi-context-caching} and Gemini~\cite{gemini}.
%
To create position-independent caching, users can call: \texttt{generate\_context\_cache(static\_token\_chunks[]) {-> cache\_ids}}. This API accepts a list of static token chunks, pre-generates the corresponding KV cache, and returns their cache IDs. 
%
For PIC-accelerated LLM inference, users can call \texttt{chat\_completion(message\_list) -> Response}, where the message list can contain both new dynamic tokens and previously returned cache IDs, arranged in any order. This flexibility marks a key distinction from state-of-the-art prefix-based context caching approaches, such as those used in Kimi~\cite{kimi-context-caching} and Gemini~\cite{gemini-context-caching}.

%
%which accepts a list of cache IDs and dynamic tokens, goes through the \textit{KVLink} prefill, the decode stage, and returns the final response.

\if 0
\begin{align*}
\texttt{expire\_cache(cache\_ids[])}
\end{align*} accepts a list of cache IDs and deletes the corresponding pre-generated KV cache.
\fi

%\ys{we can probably move this para to later sections and point to eval on chunk granularity?}
%Despite the preceding design and implementation, \system\ supports both explicit context caching and implicit context caching. In \textbf{explicit context caching}, users are responsible for splitting static tokens into chunks, explicitly calling the context caching APIs, and indexing pre-generated KV cache by cache IDs~\cite{kimi-context-caching, gemini-context-caching}. This approach enables users to convey the semantic structure of static tokens to the system, allowing for optimizations in accuracy, storage, and latency/throughput. Since users have better knowledge of the content, they can split static tokens in ways that improve subsequent linking and maintain semantic independence. \textbf{Implicit context caching} shifts the responsibility for splitting and caching to the underlying system, which indexes pre-generated KV cache using text matching (e.g., hash-based or radix-tree-based methods)~\cite{kwon2023vllm, zheng2023sglang, hu2024memserve}. While this approach reduces users' burden, it introduces indexing overhead and may result in suboptimal splitting, potentially compromising accuracy. Thus, it presents a trade-off between ease of use and system performance.


% An extension on the OpenAI-compatible API server of vLLM,
% as well as a corresponding server, client and test suite are implemented in 1K lines of Python code.
% The LLM core with extensional \textit{link} operation (as introduced in \nameref{sec:system})
% is implemented in about 1K lines of Python (for higher-level operations) and CUDA code (for lower-level
% GPU-side operations). The remaining components and the pass of control flow information are glued 
% in about 500 lines.


% \item \texttt{expire\_cache(cache\_id)}: For the sake of garbage collection,
% this API explicitly notices \system that the KV cache located by \texttt{cache\_id} is expired.
% Then \system could reclaim resource related to \texttt{cache\_id}.
% \end{itemize}

==> tables/tbl-background-positioning.tex <==
\begin{table}[t]
\begin{tabular}{ c|c|c } 
  & \textbf{Prefix-Based} & \textbf{Position-Independent} \\ 
 \hline
 \textbf{Implicit} & vLLM, OpenAI & CacheBlend \\ 
 \hline
 \textbf{Explicit} & Kimi, Gemini & \system\ (this work) \\ 
\end{tabular}
\centering
\caption{Context Caching Categorization.
Implicit APIs refer to caching mechanisms managed by the inference engine or service provider, where the process is transparent to users. In contrast, explicit APIs give users direct control over the caching process. Prefix-based caching requires an exact match of tokens to reuse cached results, whereas position-independent caching allows the reuse of the KV cache even when the tokens differ.
}
\label{tbl-background-positioning}
\end{table}
